Deep learning for multimessenger core-collapse supernova detection

The detection of gravitational waves from core-collapse supernova (CCSN) explosions is a challenging task, yet to be achieved, in which it is key the connection between multiple messengers, including neutrinos and electromagnetic signals. In this work, we present a method for detecting these kind of signals based on machine learning techniques. We tested its robustness by injecting signals in the real noise data taken by the Advanced LIGO-Virgo network during the second observation run, O2. We trained a newly developed Mini-Inception Resnet neural network using time-frequency images corresponding to injections of simulated phenomenological signals, which mimic the waveforms obtained in 3D numerical simulations of CCSNe. With this algorithm we were able to identify signals from both our phenomenological template bank and from actual numerical 3D simulations of CCSNe. We computed the detection efficiency versus the source distance, obtaining that, for signal to noise ratio higher than 15, the detection efficiency is 70 % at a false alarm rate lower than 5%. We notice also that, in the case of O2 run, it would have been possible to detect signals emitted at 1 kpc of distance, whilst lowering down the efficiency to 60%, the event distance reaches values up to 14 kpc.

==> validation.tex <==
% !TEX root = main.tex

\section{Test set}
\label{sec:testSet}

%
\begin{table*}
\caption{List of models of the test set used in the injections. $M_{\rm ZAMS}$ corresponds to the progenitor mass at zero-age in the main sequence (ZAMS).
Unless commented, all progenitors have solar metallicity, result in explosions and their GW signal do not show signatures of the standing-shock accretion
instability (SASI). }
\label{tab:SNModels}
\begin{tabular}{cccc}
\hline
Model name & reference & $M_{\rm ZAMS}$& comments\\ 
\hline
s9 & \cite{Radice_2019} & $9 M_\odot$ & Low mass progenitor, low GW amplitude. \\
s25 &\cite{Radice_2019} & $25 M_\odot$ & Develops SASI.\\
s13 &\cite{Radice_2019} & $13 M_\odot$ & Non-exploding model.\\
s18 & \cite{Powell_2018} & $18 M_\odot$ & Higher GW amplitude. \\
he3.5 & \cite{Powell_2018} & - & Ultra-stripped progenitor ($3.5 M_\odot$ He core).\\
SFHx & \cite{Kuroda_2016} & $15 M_\odot$ & Non-exploding model. Develops SASI.\\
mesa20 & \cite{O_Connor_2018} & $20 M_\odot$& \\
mesa20\_pert & \cite{O_Connor_2018} & $20 M_\odot$ & Same as mesa20, but including perturbations.\\
s11.2 & \cite{Andresen2017} & $11.2 M_\odot$ &\\
L15 & \cite{Muller2012} & $15 M_\odot$ & Simplified neutrino treatment.\\ 
\hline
\end{tabular}
\end{table*}
%
For the final test we perform injections using CCSN waveforms from numerical simulations found in the literature. In particular we focus on 
3D simulations of non-rotating progenitors representative of the neutrino driven mechanism. The selection ({\it test set}, hereafter, see Table~\ref{tab:SNModels}) is performed based on the realism of the
simulations (in terms of neutrino transport and equation of state) and on the completeness of the GW signal computed (some of the models in the literature
 compute less than $100$~ms after bounce or have a poor sampling rate). The selection includes models with a variety of mass progenitors and features
in the GW spectrum, and coincides with the choice for ongoing SN searches by the LVK collaboration. Except for model L15, non of the models coincide with the models
selected for the waveform calibration set used in Sect.~\ref{sec:waveforms}. With this choice the injected waveforms are in practice completely uncorrelated to any information 
we have used to train the CNN network.
The injection procedure is similar to the one used for the Blind set of the previous test: we inject waveforms uniformly in distance and sky directions, from 100 pc to 15 kpc.
